Automated cross-sectional view selection in CT angiography of aortic dissections with uncertainty awareness and retrospective clinical annotations

Objective: Surveillance imaging of chronic aortic diseases, such as dissections, relies on obtaining and comparing cross-sectional diameter measurements at predefined aortic landmarks, over time. Due to a lack of robust tools, the orientation of the cross-sectional planes is defined manually by highly trained operators. We show how manual annotations routinely collected in a clinic can be efficiently used to ease this task, despite the presence of a non-negligible interoperator variability in the measurements. Impact: Ill-posed but repetitive imaging tasks can be eased or automated by leveraging imperfect, retrospective clinical annotations. Methodology: In this work, we combine convolutional neural networks and uncertainty quantification methods to predict the orientation of such cross-sectional planes. We use clinical data randomly processed by 11 operators for training, and test on a smaller set processed by 3 independent operators to assess interoperator variability. Results: Our analysis shows that manual selection of cross-sectional planes is characterized by 95% limits of agreement (LOA) of $10.6^\circ$ and $21.4^\circ$ per angle. Our method showed to decrease static error by $3.57^\circ$ ($40.2$%) and $4.11^\circ$ ($32.8$%) against state of the art and LOA by $5.4^\circ$ ($49.0$%) and $16.0^\circ$ ($74.6$%) against manual processing. Conclusion: This suggests that pre-existing annotations can be an inexpensive resource in clinics to ease ill-posed and repetitive tasks like cross-section extraction for surveillance of aortic dissections.

==> comparison_krissian.tex <==
\begin{table*}
    \centering
    \caption{%
       Evaluation of the plain CNN predictions on the 12 test volumes with segmentation and interoperator variability. All errors are averaged among the three operators. For a comparison with the available literature, we also compare the centerline approaches of \cite{hahn_2020} (Hahn) and \cite{Krissian_2014} (Krissian) against the three operators. The clinical landmarks marked with * are susceptible to a higher variability due to their ill-posed nature, as shown also in \autoref{fig:landmark_pos}. 
    }
    \begin{minipage}[t]{0.95\columnwidth}
    \tabulinesep=_2pt^2pt
    \label{tab:cnn_centerline_comp}

    \begin{tabu} to \columnwidth
    {X[2cp]X[1cp]X[3cp]X[3cp]}
        \tabucline[0.10em black]-
        \textbf{Landmark} & \textbf{Method} & $\theta$-MAE [deg] & $\phi$-MAE [deg] \\
        \tabucline[0.10em black]-
        Aortic & \textbf{NoUQ}  & $\mathbf{4.38}$ & $\mathbf{6.94}$ \\
        %& Hahn & - - - & $14.82$ & $18.91$\\
        Annulus        & Krissian & $21.80 \pm 8.53$ & $26.08 \pm 20.00$ \\       
        (Ann)       & Hahn & N/A & N/A\\
        \tabucline[0.05em black!30]-
         Sinuses of & \textbf{NoUQ} & $\mathbf{3.32}$ & $\mathbf{9.07}$ \\
         Valsalva       & Krissian & $18.09 \pm 11.90$ & $34.80 \pm 18.76$\\ 
        (SoV) & Hahn & $11.51$ & $19.68$\\
        \tabucline[0.05em black!30]-
        Sinotubular & \textbf{NoUQ} & $\mathbf{2.30}$ & $\mathbf{11.74}$ \\
          Junction      & Krissian & $19.41 \pm 16.07$ & $21.24 \pm 19.68$\\ 
         (Stj)    & Hahn & $9.05$ & $19.46$\\
        \tabucline[0.05em black!30]-
        Mid  & \textbf{NoUQ} & $\mathbf{4.87}$ & $\mathbf{15.31}$ \\
          Ascending      & Krissian & $14.96 \pm 12.53$ & $19.05 \pm 13.53$\\ 
        A. (MAs)    & Hahn & $12.64$ & $21.72$\\
        \tabucline[0.05em black!30]-
        Proximal   & \textbf{NoUQ} &  $\mathbf{6.24}$ & $17.86$ \\
         Arch          & Krissian & $18.29 \pm 11.50$ & $18.59 \pm 12.37$\\ 
        (PAr)    & Hahn & $10.38$ & $\mathbf{17.34}$\\
        \tabucline[0.05em black!30]-
        Distal & NoUQ & $12.55$ & $10.23$ \\
        Arch & \textbf{Krissian} & $10.74 \pm 11.98$ & $\mathbf{7.45 \pm 7.08}$\\ 
        (DAr) & Hahn & $\mathbf{9.36}$ & $10.53$\\
%\tabucline[0.10em black]-
%\end{tabu}
%    \end{minipage}\hfill
%    \begin{minipage}[t]{\columnwidth}
%        \label{tab:cnn_centerline_comp2}
%    \tabulinesep=_3pt^3pt
%    \begin{tabu} to \columnwidth
%    {X[2cp]X[1cp]X[3cp]X[3cp]}
%        \tabucline[0.10em black]-
%        \textbf{Landmark} & \textbf{Method}
%        & $\theta$-MAE [deg] & $\phi$-MAE [deg] \\
\tabucline[0.05em black!30]-
        %\tabucline[0.10em black]-
        Proximal & NoUQ & $11.67$ & $21.81$ \\
        Descending       & Krissian & $10.86 \pm 8.11$ & $7.74 \pm 5.97$\\ 
        A. (PDe)* & \textbf{Hahn} & $\mathbf{9.21}$ & $\mathbf{6.30}$\\
        \tabucline[0.05em black!30]-
        Distal & NoUQ  & $6.62$ & $19.82$ \\
        Descending        & Krissian & $9.57\pm7.18$ & $16.22\pm14.36$\\ 
        A. (DDe)* & \textbf{Hahn} & $\mathbf{5.68}$ & $\mathbf{9.99}$\\
        \tabucline[0.05em black!30]-
        A. at celiac & NoUQ & $\mathbf{3.89}$ & $33.95$ \\
        artery & Krissian & $13.52\pm10.42$ & $34.37\pm15.49$\\ 
        (Cel) & \textbf{Hahn} & $4.99$ & $\mathbf{16.44}$\\
        \tabucline[0.05em black!30]-
        A. at inf. &  \textbf{NoUQ}  & $\mathbf{3.93}$ & $26.86$ \\
        main renal & Krissian & $7.07\pm5.70$ & $\mathbf{22.21\pm14.23}$\\ 
        art. (Ren) & {Hahn}  & $4.82$ & ${24.30}$\\
        \tabucline[0.05em black!30]-
        Above &  \textbf{NoUQ} & $\mathbf{4.03}$ & $\mathbf{9.35}$ \\
        iliac bifur. & Krissian* & $11.21\pm 7.17$ & $23.05 \pm 14.55$\\ 
        (Bif) & Hahn & $11.19$ & $20.61$\\
        \tabucline[0.05em black!30]-
        \textbf{Overall}    & \textbf{NoUQ} &  $\mathbf{5.80}$ & $\mathbf{16.63}$ \\
        (All) & Krissian* & $14.21 \pm 11.44$ & $21.01 \pm 17.11$\\ 
         & Hahn  & $8.88$ & $16.64$\\
        \tabucline[0.10em black]-

    \end{tabu}
    \end{minipage}
\end{table*}
